Towards Low-Latency and Energy-Efficient Hybrid P2P-CDN Live Video Streaming

Streaming segmented videos over the Hypertext Transfer Protocol (HTTP) is an increasingly popular approach in both live and video-on-demand (VoD) applications. However, designing a scalable and adaptable framework that reduces servers energy consumption and supports low latency and high quality services, particularly for live video streaming scenarios, is still challenging for Over-The-Top (OTT) service providers. To address such challenges, this paper introduces a new hybrid P2P-CDN framework that leverages new networking and computing paradigms, i.e., Network Function Virtualization (NFV) and edge computing for live video streaming. The proposed framework introduces a multi-layer architecture and a tree of possible actions therein (an action tree), taking into account all available resources from peers, edge, and CDN servers to efficiently distribute video fetching and transcoding tasks across a hybrid P2P-CDN network, consequently enhancing the users latency and video quality. We also discuss our testbed designed to validate the framework and compare it with baseline methods. The experimental results indicate that the proposed framework improves user Quality of Experience (QoE), reduces client serving latency, and improves edge server energy consumption compared to baseline approaches.

==> IEEE_MMTC_Frontiers_Arxiv/Bio.tex <==
\vspace{-1cm}
\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorsPics/Reza.jpg}}]
{Reza Farahani} is a Postdoctoral researcher at the Institute of Information Technology (ITEC), University of Klagenfurt. He received his Ph.D. and M.Sc degrees in information technology and computer engineering in 2023 and 2019, respectively, from the University of Klagenfurt, Klagenfurt, Austria, and the University of Tehran, Tehran, IRAN. Between October 2019 and February 2023, he was involved in the ATHENA project, funded by the Christian Doppler Forschungsgesellschaft and the industry partner Bitmovin GmbH. From November 2022 to January 2023, he was a visiting scholar at the 5G\&6G Innovation Centre (5GIC\&6GIC), Institute for Communication Systems (ICS), at the University of Surrey, UK. He has co-authored more than 25 publications in international conferences and journals. Additionally, he has held the role of technical program chair for several international conferences. He has also been working in the computer networks field in different roles, e.g.,  network engineer, developer, protocol designer, and instructor (R\&S, SP) for over six years. His research interests are Network and Service Management, Parallel and Distributed Systems, Multimedia Communication, Edge-Cloud Continuum, Serverless Computing, Network Softwarization/Virtualization, Mathematics Optimization, and Distributed Learning approaches. 
\end{IEEEbiography}
%%%%%%%%%
\vspace{-1cm}
\begin{IEEEbiography} 
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorsPics/Christian.jpeg}}]
{Christian Timmerer}\textbf{(M'08-SM'16)} is a full professor of computer science at Alpen-Adria-Universität Klagenfurt (AAU), Institute of Information Technology (ITEC), and he is the director of the Christian Doppler (CD) Laboratory ATHENA (\url{https://athena.itec.aau.at/}). His research interests include multimedia systems, immersive multimedia communication, streaming, adaptation, and quality of experience where he co-authored eight patents and more than 300 articles. He was the general chair of WIAMIS 2008, QoMEX 2013, MMSys 2016, and PV 2018 and has participated in several EC-funded projects, notably DANAE, ENTHRONE, P2P-Next, ALICANTE, SocialSensor, COST IC1003 QUALINET, ICoSOLE, and SPIRIT. He also participated in ISO/MPEG work for several years, notably in MPEG-21, MPEG-M, MPEG-V, and MPEG-DASH, where he served as standard editor. In 2012 he cofounded Bitmovin (\url{http://www.bitmovin.com/}) to provide professional services around MPEG-DASH, where he holds the position of the Chief Innovation Officer (CIO) -- Head of Research and Standardization. Further information at \url{http://timmerer.com}. 
\end{IEEEbiography}
%%%%%%%%%%%
\vspace{-.5cm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorsPics/Hermann.pdf}}]
{Hermann Hellwagner} 
is a full professor of computer science at Alpen-Adria-Universität Klagenfurt (AAU) where he leads the research group Multimedia Communication (MMC) in the Institute of Information Technology (ITEC). Earlier, he held positions as an associate professor at the University of Technology in Munich (TUM) and as a senior researcher at Siemens Corporate Research in Munich. His current research areas are distributed multimedia systems, multimedia communication and adaptation, QoS/QoE, and communication in multi-UAV networks. He has published widely on parallel computer architecture, parallel programming, and multimedia communication and adaptation. He is a senior member of the IEEE and of the ACM. He was a member of the Scientific Board of the Austrian Science Fund (FWF) (2005-2016) and an FWF Vice President (2013–2016). Currently, he is a member of the CD Senate of Christian Doppler Forschungsgesellschaft (CDG). Further information at \url{https://www.itec.aau.at/~hellwagn/}.
\end{IEEEbiography}


